Distributed Quantum Computing Utilizing Multiple Codes on Imperfect Hardware

Quantum bits have technological imperfections. Additionally, the capacity of a component that can be implemented feasibly is limited. Therefore, distributed quantum computation is required to scale up quantum computers. This dissertation presents a new quantum computer architecture which takes into account imperfections, aimed to realize distributed computation by connecting quantum computers each of which consists of multiple quantum CPUs and memories. Quantum CPUs employ a quantum error correcting code which has faster logical gates and quantum memories employ a code which is superior in space resource requirements. This dissertation focuses on quantum error correcting codes, giving a practical, concrete method for tolerating static losses such as faulty devices for the surface code. Numerical simulation with practical assumptions showed that a yield of functional qubits of 90% is marginally capable of building large-scale systems, by culling the poorer 50% of lattices during post-fabrication testing. Yield 80% is not usable even when culling 90% of generated lattices. For internal connections in a quantum computer and for connections between quantum computers, this dissertation gives a fault-tolerant method that bridges heterogeneous quantum error correcting codes. Numerical simulation showed that the scheme, which discards any quantum state in which any error is detected, always achieves an adequate logical error rate regardless of physical error rates in exchange for increased resource consumption. This dissertation gives a new extension of the surface code suitable for memories. This code is shown to require fewer physical qubits to encode a logical qubit than conventional codes. This code achieves the reduction of 50% physical qubits per a logical qubit. Collectively, the elements to propose the distributed quantum computer architecture are brought together.

==> glossaries_db.tex <==
\newglossaryentry{EMTD}{
name=Extended MANEMO Tree Discovery,
description={ (EMTD) is a simple distance vector protocol built on
the Router Advertisement message of the Neighbor Discovery
protocol~\cite{rfc4861}. It is an extension of existing protocols: Tree
Discovery protocol (TDP)~\cite{td-draft} with Network In Node
Advertisement (NINA)~\cite{nina-draft}}
}

\newacronym[description= Extended MANEMO Tree Discovery: is a simple
distance vector protocol built on the Router Advertisement message of
the Neighbor Discovery protocol~\cite{rfc4861}. It is an extension of
existing protocols: Tree Discovery protocol (TDP)~\cite{td-draft} with
Network In Node Advertisement
(NINA)~\cite{nina-draft}]{emtd}{EMTD}{Extended MANEMO Tree Discovery}



\newglossaryentry{Mobile Router}{
name=Mobile Router,
description={As defined in ~\cite{rfc3753}: A router capable of Network
Mobility (RFC3963~\cite{rfc3963}) to provide group mobility to Mobile
Network Node in mobile network}
}

\newglossaryentry{Floating Router}{
name=Floating Router,
description={is a kind of Mobile Router that has a capability of joining
Floating Ground}
}

\newglossaryentry{Root Floating Router}{
name=Root Floating Router,
description={is a Floating Router that has direct connectivity to Access Router}
}

\newglossaryentry{Floating Ground}{
name=Floating Ground,
description={is a logical component provides overlay network
between access network and mobile network}
}
%\newacronym{Floating Ground}{\glsadd{floating ground}FG}{Floating Ground}

\newglossaryentry{Floating Ground Architecture}{
name=Floating Ground Architecture,
description={ (FGA) is a network architecture that enables to integrate any two
different network system with Floating Ground as a buffer layer}
}

\newacronym[description={Direct Code Execution: refers to the ability of
a simulator to execute directly within itself in simulated time an
program that was not originally developed to be run in a
simulator~\cite{lacage2010phd}}]{dce}{DCE}{Direct Code Execution}

\newglossaryentry{topologically correct address}{
name=Topologically Correct Address,
description={is a address that represents correct location in the
network topology}
}

\newglossaryentry{topologically incorrect address}{
name=Topologically Incorrect Address,
description={is a address that does not represent correct location in the
network topology. The example is Provider Independent address (PI)}
}

\newacronym[description={MANET for NEMO: is the solution that combines
two existing technologies to solve the problems of both MANET and
NEMO}]{MANEMO}{MANEMO}{MANET for NEMO}

\newglossaryentry{Mobile Host}{name=Mobile Host,description={}}
\newglossaryentry{Host}{name=Host,description={}}
\newglossaryentry{Router}{name=Router,description={}}
\newglossaryentry{Node}{name=Node,description={}}
\newglossaryentry{Fixed Internet}{name=Fixed Internet,description={}}
\newglossaryentry{Mobile Node/MNN/MNP/HA/MH}{name=Mobile Node/MNN/MNP/HA/MH,description={}}
\newglossaryentry{MANEMO Fringe Stub/Fringe Stub}{name=MANEMO Fringe Stub/Fringe Stub,description={}}
\newglossaryentry{Network Extension}{name=Network Extension,description={}}
\newglossaryentry{Network Attachment}{name=Network Attachment,description={}}


